The Value of Information When Deciding What to Learn

All sequential decision-making agents explore so as to acquire knowledge about a particular target. It is often the responsibility of the agent designer to construct this target which, in rich and complex environments, constitutes a onerous burden; without full knowledge of the environment itself, a designer may forge a sub-optimal learning target that poorly balances the amount of information an agent must acquire to identify the target against the target's associated performance shortfall. While recent work has developed a connection between learning targets and rate-distortion theory to address this challenge and empower agents that decide what to learn in an automated fashion, the proposed algorithm does not optimally tackle the equally important challenge of efficient information acquisition. In this work, building upon the seminal design principle of information-directed sampling (Russo & Van Roy, 2014), we address this shortcoming directly to couple optimal information acquisition with the optimal design of learning targets. Along the way, we offer new insights into learning targets from the literature on rate-distortion theory before turning to empirical results that confirm the value of information when deciding what to learn.

==> Blahut-Arimoto + IDS/commands.tex <==
% Dynamically sized mid bar.
\newcommand{\bigmid}{\mathrel{\Big|}}

% ---- Colors and Notes ----
\definecolor{dblue}{RGB}{98, 140, 190}
\definecolor{dlblue}{RGB}{216, 235, 255}
\definecolor{dgreen}{RGB}{124, 155, 127}
\definecolor{dpink}{RGB}{207, 166, 208}
\definecolor{dyellow}{RGB}{255, 248, 199}
\definecolor{dgray}{RGB}{46, 49, 49}

% URL
\newcommand{\durl}[1]{\textcolor{dblue}{\underline{\url{#1}}}}

% Circled Numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.7pt] (char) {\footnotesize{#1}};}}
% From: http://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers

% Under set numbered subset of equation
\newcommand{\numeq}[3]{\underset{\textcolor{#2}{\circled{#1}}}{\textcolor{#2}{#3}}}

% ---- Abbreviations -----
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\ubr}[1]{\underbrace{#1}}
\newcommand{\uset}[2]{\underset{#1}{#2}}
\newcommand{\eps}{\varepsilon}
\newcommand{\del}{\delta}

% Typical limit:
\newcommand{\nlim}{\underset{n \rightarrow \infty}{\lim}}
\newcommand{\nliminf}{\liminf\limits_{n \rightarrow \infty}}
\newcommand{\nlimsup}{\limsup\limits_{n \rightarrow \infty}}
\newcommand{\nsum}{\sum_{i = 1}^n}
\newcommand{\nprod}{\prod_{i = 1}^n}

% Add an hrule with some space
\newcommand{\spacerule}{\begin{center}\hdashrule{2cm}{1pt}{1pt}\end{center}}

% Mathcal and Mathbb
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\indic}{\mathbbm{1}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\rank}{\text{rank}}
\newcommand{\kl}[2]{D_{\mathrm{KL}}(#1\text{ }||\text{ }#2)}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\variance}[1]{\mathbb{V}\left[#1\right]}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\covar}[1]{Cov\left[#1\right]}
\newcommand{\dlog}[1]{\log\left(#1\right)}
\newcommand{\dexp}[1]{\exp\left(#1\right)}
\newcommand{\dell}{\dot{\ell}}
\newcommand{\ddell}{\ddot{\ell}}
\newcommand{\pdot}{\dot{p}}
\newcommand{\sdot}{\dot{s}}
\newcommand{\diam}[1]{\text{diam}\left(#1\right)}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\card}[1]{\text{card}\left(#1\right)}
\newcommand{\trace}[1]{\text{trace}\left(#1\right)}
\newcommand{\sign}[1]{\text{sign}\left(#1\right)}
\newcommand{\oover}[1]{\frac{1}{#1}}

\DeclareMathOperator*{\esssup}{ess\,sup}

\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\da}{\downarrow}
\newcommand{\ua}{\uparrow}

\newcommand{\sigalg}{$\sigma$-algebra}
\newcommand{\sigfin}{$\sigma$-finite}
\newcommand{\sig}{$\sigma$}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\om}{\Omega}
\newcommand{\lamsys}{$\lambda$-system}
\newcommand{\pisys}{$\pi$-system}
\newcommand{\holder}{H\"older's }
\newcommand{\arzela}{Arzel\'a}
\newcommand{\cadlag}{c\'adl\'ag }
\newcommand{\pspace}{(\Omega,\mc{F},\bP)}
\newcommand{\lp}[2]{\Big|\Big|#2\Big|\Big|_{L^{#1}}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\vol}[1]{\text{Vol}\left(#1\right)}
\newcommand{\borel}[1]{\mc{B}(#1)}
\newcommand{\sfp}{\text{SF}^+}
\newcommand{\sfpf}[1]{\text{SF}^+(#1)}
\newcommand{\pos}[1]{#1^+}
\newcommand{\negt}[1]{#1^-}
\newcommand{\dsum}[3]{\sum\limits_{#1=#2}^{#3}}
\newcommand{\disum}[2]{\sum\limits_{i=#1}^{#2}}
\newcommand{\djsum}[2]{\sum\limits_{j=#1}^{#2}}
\newcommand{\dnsum}[2]{\sum\limits_{n=#1}^{#2}}
\newcommand{\ale}{\text{ a.e.}}
\newcommand{\io}{\text{ i.o.}}
\newcommand{\cov}{\text{Cov}}
\newcommand{\infint}{\int\limits_{-\infty}^\infty}
\newcommand{\dprod}[3]{\prod\limits_{#1=#2}^{#3}}
\newcommand{\diprod}[2]{\prod\limits_{i=#1}^{#2}}
\newcommand{\djprod}[2]{\prod\limits_{j=#1}^{#2}}
\newcommand{\dnprod}[2]{\prod\limits_{n=#1}^{#2}}
\newcommand{\timesdots}{\times \ldots \times}
\newcommand{\cylomega}[1]{\Omega^{(#1)}}
\newcommand{\Perp}{\perp \! \! \! \perp}
\newcommand{\dcon}{\overset{d}{\rightarrow}}
\newcommand{\pcon}{\overset{p}{\rightarrow}}
\newcommand{\ascon}{\overset{a.s.}{\rightarrow}}
\newcommand{\lpcon}{\overset{L^p}{\rightarrow}}
\newcommand{\aseq}{\overset{a.s.}{=}}
\newcommand{\deq}{\overset{d}{=}}
\newcommand{\astext}{\text{ as }}
\newcommand{\iid}{\overset{i.i.d.}{\sim}}
\newcommand{\psd}{\succeq}
\newcommand{\pd}{\succ}
\newcommand{\lop}{o_p}
\newcommand{\bop}{\mathcal{O}_p}
\newcommand{\grad}{\nabla}
\newcommand{\esttheta}{\widehat{\theta}}
\newcommand{\estthetan}{\widehat{\theta}_n}
\newcommand{\sqn}{\sqrt{n}}
\newcommand{\hsqn}{\frac{h}{\sqrt{n}}}
\newcommand{\samsum}{\frac{1}{n}\sum\limits_{i=1}^n}
\newcommand{\supfun}{\sup\limits_{f \in \mathcal{F}}}
\newcommand{\inffun}{\inf\limits_{f \in \mathcal{F}}}
\newcommand{\pno}{P_n^0}
\newcommand{\vc}{\text{VC}}
\newcommand{\vcc}{\vc(\mc{C})}
\newcommand{\dpq}{\frac{dP_n}{dQ_n}}
\newcommand{\dqp}{\frac{dQ_n}{dP_n}}

% argmin, argmax.
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% ---- Figures, Boxes, Theorems, Etc. ----

% Basic Image
\newcommand{\img}[2]{
\begin{center}
\includegraphics[scale=#2]{#1}
\end{center}}

% Put a fancy box around things.
\newcommand{\dbox}[1]{
\begin{mdframed}[roundcorner=4pt, backgroundcolor=gray!5]
\vspace{1mm}
{#1}
\end{mdframed}
}

%  --- PROOFS ---

% Inner environment for Proofs
\newmdenv[
  topline=false,
  bottomline=false,
  rightline = false,
  leftmargin=10pt,
  rightmargin=0pt,
  innertopmargin=0pt,
  innerbottommargin=0pt
]{innerproof}

% Proof Command
%\newenvironment{dproof}{\begin{proof} \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}
\newenvironment{dproof}[1][Proof]{\begin{proof}[#1] \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}


% Dave Definition
\newcounter{DaveDefCounter}
\setcounter{DaveDefCounter}{1}

\newcommand{\ddef}[2]
{
\begin{mdframed}[roundcorner=1pt, backgroundcolor=white]
\vspace{1mm}
{\bf Definition \theDaveDefCounter} (#1): {\it #2}
\stepcounter{DaveDefCounter}
\end{mdframed}
}

% Block Quote
\newenvironment{dblockquote}[2]{
\begin{blockquote}
#2
\vspace{-2mm}\hspace{10mm}{#1} \\
\end{blockquote}}

% Algorithm
\newenvironment{dalg}[1]
{\begin{algorithm}\caption{#1}\begin{algorithmic}}
{\end{algorithmic}\end{algorithm}}

% Dave Table
\newenvironment{dtable}[1]
{\begin{figure}[h]
\centering
\begin{tabular}{#1}\toprule}
{\bottomrule
\end{tabular}
\end{figure}}

% For numbering the last of an align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{fact}{Fact}
\newtheorem{question}{Question}

==> Blahut-Arimoto + IDS/proofs_neurips/blahut_arimoto_proof.tex <==
\begin{dproof}
For the first inequality, recall that $\bP_\chi$ is the true marginal distribution over learning targets induced by $\bP_{\environment,\chi}$. Moreover, by definition, we have that $$\mc{J}(\bP_{\environment, \chi}, \bP_{\chi}, \beta) = D_\text{KL}(\bP_{\environment, \chi} || \bP_{\environment} \times \bP_{\chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] = \bI(\environment; \chi) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)].$$ Therefore, by Fact \ref{fact:mi_inf}, it follows that $$\mc{J}(\bP_{\environment, \chi}, \bQ_{\chi}, \beta) = \mc{J}(\bP_{\environment, \chi}, \bP_{\chi}, \beta) + \kl{\bP_\chi}{\bQ_\chi}.$$ The inequality then follows immediately by Fact \ref{fact:gibbs}.

For the second inequality, we have 
\begin{align*}
    \mc{J}(&\bP_{\environment,\chi}, \bQ_\chi, \beta) = \kl{\bP_{\environment,\chi}}{\bP_\environment \times \bQ_\chi} + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\exp\left(-\beta d(\environment,\chi)\right)\right) d\bP_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\alpha_{\bQ_{\chi},\beta}(\environment) \exp\left(-\beta d(\environment,\chi)\right)\right) d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\frac{d\bQ_{\environment,\chi}}{d\bP_{\environment} \times \bQ_{\chi}}(\environment,\chi)\right) d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\cdot \frac{d\bP_{\environment} \times \bQ_{\chi}}{d\bQ_{\environment,\chi}}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bQ_{\environment,\chi}}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)
\end{align*}
where the sixth line employs the chain rule for Radon-Nikodym derivatives (Fact \ref{fact:rn_chain}). Expanding the second term and using the fact marginal distribution over $\environment$ induced by $\bQ_{\environment,\chi}$ is the same as $\bP_{\environment}$, we have
\begin{align*}
    \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment) &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bQ_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\exp\left(-\beta d(\environment,\chi)\right)\exp\left(\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\exp\left(-\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi) + \int \log\left(\exp\left(\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi)\\
    &= \int \log\left(\frac{d\bQ_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right) d\bQ_{\environment,\chi}(\environment,\chi) + \beta \int d(\environment,\chi)  d\bQ_{\environment,\chi}(\environment,\chi)\\
    &= \kl{\bQ_{\environment,\chi}}{\bP_\environment \times \bQ_\chi} + \beta \bE_{\bQ_{\environment,\chi}}\left[d(\environment,\chi)\right] \\
    &= \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta)
\end{align*}
Substituting back and applying Fact \ref{fact:gibbs} once more yields the inequality
\begin{align*}
    \mc{J}(\bP_{\environment,\chi}, \bQ_\chi, \beta) &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment) \\
    &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta) \\
    &\geq \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta)
\end{align*}
\end{dproof}

==> Blahut-Arimoto + IDS/proofs_neurips/rd_slope_proof.tex <==
\begin{dproof}
The correspondence between values of $\beta$ and values of $D$ is a geometric argument. We have that for any fixed $D \geq 0$ and for all $\beta \geq 0$,
\begin{align*}
    \mc{R}(D) &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \bI(\bP_{\environment, \chi}) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)]  - \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) \\
    &\geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) - \beta D \\
    &\geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) - \beta D \\
    &= \mc{F}(\beta) - \beta D
\end{align*}
This inequality coupled with the fact that $\mc{R}(D)$ is convex implies the existence of a straight line with slope $\beta_D$ passing through the point $(D,\mc{R}(D))$ such that $\mc{F}(\beta) - \beta_D D = \mc{R}(D)$ with no points above the rate-distortion curve. Consequently, the notion of a particular $\beta_D$ associated with $D$ implies that for all $D'$, $$\mc{R}(D') + \beta_D D' \geq \mc{R}(D) + \beta_D D.$$

To see that this lower bound is achieved by the $\beta_D$ value associated with a given threshold $D$, let $\bP_{\environment,\chi}$ be a joint distribution with expected distortion $D'$ such that for $\eps > 0$, $$\bI(\bP_{\environment,\chi}) + \beta_D \bE_{\environment,\chi}[d(\environment,\chi)] \leq \mc{F}(\beta_D) + \eps.$$ Using the previous two inequalities, we have 
\begin{align*}
    \mc{F}(\beta_D) + \eps \geq \mc{R}(D') + \beta_D D' \geq \mc{R}(D) + \beta_D D &\geq \mc{F}(\beta_D)
\end{align*}
Since our choice of $\eps$ was arbitrary, taking the limit as $\eps \ra 0$ yields $$\mc{F}(\beta_D) = \mc{R}(D) + \beta_D D.$$

Notably, the Blahut-Arimoto algorithm for computing rate-distortion functions operates with a specification of $\beta$, rather than $D$. Let $\bP_{\environment,\chi}^\star$ be the joint distribution such that $$\mc{F}(\beta) = \inf\limits_{\bP_{\environment,\chi} \in \Lambda} \left(\bI(\bP_{\environment,\chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)]\right) = \bI(\bP_{\environment,\chi}^\star) + \beta \bE_{\bP_{\environment,\chi}^\star}[d(\environment,\chi)].$$ Defining $D_\beta = \bE_{\bP_{\environment,\chi}^\star}[d(\environment,\chi)]$ and $R_\beta = \bI(\bP_{\environment,\chi}^\star)$, we have the lower bound $$\mc{F}(\beta) = R_\beta + \beta D_\beta \geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \bI(\bP_{\environment, \chi}) + \beta D_\beta = \mc{R}(D_\beta) + \beta D_\beta.$$ For the upper bound, we have 
\begin{align*}
    \mc{F}(\beta) &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda} \left(\bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)] \right) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \left(\bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)]\right) \\
    &\leq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \left(\bI(\bP_{\environment, \chi}) + \beta D_\beta \right) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \bI(\bP_{\environment, \chi}) + \beta D_\beta \\ 
    &= \mc{R}(D_\beta) + \beta D_\beta
\end{align*}
Putting both inequalities together shows that $\mc{F}(\beta) = \mc{R}(D_\beta) + \beta D_\beta$, which implies that $\beta$ is associated with $D_\beta$ and $\mc{R}(D_\beta) = \mc{F}(\beta) - \beta D_\beta$.
\end{dproof}

==> proofs_neurips/blahut_arimoto_proof.tex <==
\begin{dproof}
For the first inequality, recall that $\bP_\chi$ is the true marginal distribution over learning targets induced by $\bP_{\environment,\chi}$. Moreover, by definition, we have that $$\mc{J}(\bP_{\environment, \chi}, \bP_{\chi}, \beta) = D_\text{KL}(\bP_{\environment, \chi} || \bP_{\environment} \times \bP_{\chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] = \bI(\environment; \chi) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)].$$ Therefore, by Fact \ref{fact:mi_inf}, it follows that $$\mc{J}(\bP_{\environment, \chi}, \bQ_{\chi}, \beta) = \mc{J}(\bP_{\environment, \chi}, \bP_{\chi}, \beta) + \kl{\bP_\chi}{\bQ_\chi}.$$ The inequality then follows immediately by Fact \ref{fact:gibbs}.

For the second inequality, we have 
\begin{align*}
    \mc{J}(&\bP_{\environment,\chi}, \bQ_\chi, \beta) = \kl{\bP_{\environment,\chi}}{\bP_\environment \times \bQ_\chi} + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\exp\left(-\beta d(\environment,\chi)\right)\right) d\bP_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\alpha_{\bQ_{\chi},\beta}(\environment) \exp\left(-\beta d(\environment,\chi)\right)\right) d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) - \int \log\left(\frac{d\bQ_{\environment,\chi}}{d\bP_{\environment} \times \bQ_{\chi}}(\environment,\chi)\right) d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\cdot \frac{d\bP_{\environment} \times \bQ_{\chi}}{d\bQ_{\environment,\chi}}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \int \log\left(\frac{d\bP_{\environment,\chi}}{d\bQ_{\environment,\chi}}(\environment,\chi)\right)d\bP_{\environment,\chi}(\environment,\chi) + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)\\
    &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment)
\end{align*}
where the sixth line employs the chain rule for Radon-Nikodym derivatives (Fact \ref{fact:rn_chain}). Expanding the second term and using the fact marginal distribution over $\environment$ induced by $\bQ_{\environment,\chi}$ is the same as $\bP_{\environment}$, we have
\begin{align*}
    \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment) &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bQ_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\exp\left(-\beta d(\environment,\chi)\right)\exp\left(\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi) \\
    &= \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\exp\left(-\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi) + \int \log\left(\exp\left(\beta d(\environment,\chi)\right)\right) d\bQ_{\environment,\chi}(\environment,\chi)\\
    &= \int \log\left(\frac{d\bQ_{\environment,\chi}}{d\bP_\environment \times \bQ_\chi}(\environment,\chi)\right) d\bQ_{\environment,\chi}(\environment,\chi) + \beta \int d(\environment,\chi)  d\bQ_{\environment,\chi}(\environment,\chi)\\
    &= \kl{\bQ_{\environment,\chi}}{\bP_\environment \times \bQ_\chi} + \beta \bE_{\bQ_{\environment,\chi}}\left[d(\environment,\chi)\right] \\
    &= \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta)
\end{align*}
Substituting back and applying Fact \ref{fact:gibbs} once more yields the inequality
\begin{align*}
    \mc{J}(\bP_{\environment,\chi}, \bQ_\chi, \beta) &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \int \log\left(\alpha_{\bQ_\chi,\beta}(\environment)\right) d\bP_{\environment}(\environment) \\
    &= \kl{\bP_{\environment,\chi}}{\bQ_{\environment,\chi}} + \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta) \\
    &\geq \mc{J}(\bQ_{\environment,\chi}, \bQ_{\chi}, \beta)
\end{align*}
\end{dproof}

==> proofs_neurips/rd_slope_proof.tex <==
\begin{dproof}
The correspondence between values of $\beta$ and values of $D$ is a geometric argument. We have that for any fixed $D \geq 0$ and for all $\beta \geq 0$,
\begin{align*}
    \mc{R}(D) &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \bI(\bP_{\environment, \chi}) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)]  - \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) \\
    &\geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) - \beta D \\
    &\geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda} \left( \bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment, \chi}}[d(\environment, \chi)] \right) - \beta D \\
    &= \mc{F}(\beta) - \beta D
\end{align*}
This inequality coupled with the fact that $\mc{R}(D)$ is convex implies the existence of a straight line with slope $\beta_D$ passing through the point $(D,\mc{R}(D))$ such that $\mc{F}(\beta) - \beta_D D = \mc{R}(D)$ with no points above the rate-distortion curve. Consequently, the notion of a particular $\beta_D$ associated with $D$ implies that for all $D'$, $$\mc{R}(D') + \beta_D D' \geq \mc{R}(D) + \beta_D D.$$

To see that this lower bound is achieved by the $\beta_D$ value associated with a given threshold $D$, let $\bP_{\environment,\chi}$ be a joint distribution with expected distortion $D'$ such that for $\eps > 0$, $$\bI(\bP_{\environment,\chi}) + \beta_D \bE_{\environment,\chi}[d(\environment,\chi)] \leq \mc{F}(\beta_D) + \eps.$$ Using the previous two inequalities, we have 
\begin{align*}
    \mc{F}(\beta_D) + \eps \geq \mc{R}(D') + \beta_D D' \geq \mc{R}(D) + \beta_D D &\geq \mc{F}(\beta_D)
\end{align*}
Since our choice of $\eps$ was arbitrary, taking the limit as $\eps \ra 0$ yields $$\mc{F}(\beta_D) = \mc{R}(D) + \beta_D D.$$

Notably, the Blahut-Arimoto algorithm for computing rate-distortion functions operates with a specification of $\beta$, rather than $D$. Let $\bP_{\environment,\chi}^\star$ be the joint distribution such that $$\mc{F}(\beta) = \inf\limits_{\bP_{\environment,\chi} \in \Lambda} \left(\bI(\bP_{\environment,\chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)]\right) = \bI(\bP_{\environment,\chi}^\star) + \beta \bE_{\bP_{\environment,\chi}^\star}[d(\environment,\chi)].$$ Defining $D_\beta = \bE_{\bP_{\environment,\chi}^\star}[d(\environment,\chi)]$ and $R_\beta = \bI(\bP_{\environment,\chi}^\star)$, we have the lower bound $$\mc{F}(\beta) = R_\beta + \beta D_\beta \geq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \bI(\bP_{\environment, \chi}) + \beta D_\beta = \mc{R}(D_\beta) + \beta D_\beta.$$ For the upper bound, we have 
\begin{align*}
    \mc{F}(\beta) &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda} \left(\bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)] \right) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \left(\bI(\bP_{\environment, \chi}) + \beta \bE_{\bP_{\environment,\chi}}[d(\environment,\chi)]\right) \\
    &\leq \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \left(\bI(\bP_{\environment, \chi}) + \beta D_\beta \right) \\
    &= \inf\limits_{\bP_{\environment, \chi} \in \Lambda : \bE\left[d(\environment, \chi)\right] \leq D_\beta} \bI(\bP_{\environment, \chi}) + \beta D_\beta \\ 
    &= \mc{R}(D_\beta) + \beta D_\beta
\end{align*}
Putting both inequalities together shows that $\mc{F}(\beta) = \mc{R}(D_\beta) + \beta D_\beta$, which implies that $\beta$ is associated with $D_\beta$ and $\mc{R}(D_\beta) = \mc{F}(\beta) - \beta D_\beta$.
\end{dproof}
